Delving into Dark Regions for Robust Shadow Detection

Shadow detection is a challenging task as it requires a comprehensive understanding of shadow characteristics and global/local illumination conditions. We observe from our experiment that state-of-the-art deep methods tend to have higher error rates in differentiating shadow pixels from non-shadow pixels in dark regions (ie, regions with low-intensity values). Our key insight to this problem is that existing methods typically learn discriminative shadow features from the whole image globally, covering the full range of intensity values, and may not learn the subtle differences between shadow and non-shadow pixels in dark regions. Hence, if we can design a model to focus on a narrower range of low-intensity regions, it may be able to learn better discriminative features for shadow detection. Inspired by this insight, we propose a novel shadow detection approach that first learns global contextual cues over the entire image and then zooms into the dark regions to learn local shadow representations. To this end, we formulate an effective dark-region recommendation (DRR) module to recommend regions of low-intensity values, and a novel dark-aware shadow analysis (DASA) module to learn dark-aware shadow features from the recommended dark regions. Extensive experiments show that the proposed method outperforms the state-of-the-art methods on three popular shadow detection datasets. Code is available at https://github.com/guanhuankang/ShadowDetection2021.git.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> rebuttal/internet_samples.tex <==

    \includegraphics[width=0.125\linewidth]{rebuttal/internet/0_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/0_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/0_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/0_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/1_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/1_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/1_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/1_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/2_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/2_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/2_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/2_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/3_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/3_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/3_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/3_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/4_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/4_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/4_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/4_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/5_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/5_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/5_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/5_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/6_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/6_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/6_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/6_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/7_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/7_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/7_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/7_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/8_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/8_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/8_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/8_ours.jpg} & 
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/10_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/10_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/10_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/10_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/9_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/9_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/9_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/9_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/11_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/11_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/11_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/11_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/12_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/12_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/12_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/12_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/13_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/13_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/13_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/13_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/14_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/14_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/14_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/14_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/15_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/15_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/15_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/15_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/16_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/16_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/16_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/16_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/17_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/17_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/17_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/17_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/18_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/18_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/18_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/18_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/19_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/19_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/19_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/19_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/20_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/20_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/20_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/20_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/21_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/21_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/21_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/21_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/22_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/22_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/22_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/22_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/23_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/23_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/23_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/23_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/24_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/24_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/24_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/24_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/25_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/25_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/25_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/25_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/26_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/26_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/26_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/26_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/27_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/27_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/27_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/27_ours.jpg} \\
    
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/28_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/28_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/28_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/28_ours.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/29_input.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/29_bdrar.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/29_dsdnet.jpg} &
    \includegraphics[width=0.125\linewidth]{rebuttal/internet/29_ours.jpg} \\
    

==> rebuttal/synthesize_pair.tex <==

    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0071_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0071_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0071_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0075_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0075_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0075_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0076_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0076_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0076_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0090_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0090_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0090_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0092_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0092_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0092_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0097_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0097_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0097_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0099_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0099_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0099_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0113_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0113_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0113_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0114_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0114_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0114_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0120_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0120_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0120_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0122_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0122_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0122_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0123_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0123_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0123_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0127_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0127_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0127_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0128_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0128_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0128_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0129_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0129_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0129_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0141_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0141_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0141_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0143_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0143_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0143_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0144_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0144_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0144_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0148_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0148_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0148_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0150_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0150_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0150_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0152_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0152_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0152_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0157_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0157_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0157_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0159_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0159_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0159_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0161_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0161_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0161_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0163_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0163_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0163_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0164_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0164_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0164_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0165_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0165_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0165_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0166_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0166_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0166_gt.jpg} \\
    
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_gt.jpg} \\
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0248_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0248_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0248_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0261_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0261_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0261_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0262_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0262_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0262_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0272_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0272_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0272_gt.jpg} \\
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0276_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0276_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0276_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0277_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0277_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0277_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0281_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0281_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0281_gt.jpg} &
    
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_image.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_ours.jpg} &
    % \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0288_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0288_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0288_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0296_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0296_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0296_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0298_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0298_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0298_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0319_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0319_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0319_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0321_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0321_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0321_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0330_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0330_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0330_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0331_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0331_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0331_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0351_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0351_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0351_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0356_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0356_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0356_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0357_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0357_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0357_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0360_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0360_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0360_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0365_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0365_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0365_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0366_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0366_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0366_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0376_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0376_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0376_gt.jpg} \\
    

==> rebuttal/synthesize_samples.tex <==

    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0988_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0988_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0988_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0988_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0988_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1391_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1391_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1391_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1391_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1391_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1016_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1016_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1016_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1016_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1016_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1395_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1395_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1395_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1395_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1395_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1020_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1020_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1020_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1020_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1020_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1460_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1460_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1460_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1460_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1460_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1047_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1047_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1047_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1047_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1047_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1482_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1482_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1482_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1482_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1482_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1053_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1053_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1053_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1053_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1053_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1484_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1484_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1484_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1484_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1484_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1067_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1067_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1067_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1067_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1067_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1550_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1550_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1550_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1550_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1550_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1222_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1222_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1222_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1222_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1222_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1580_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1580_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1580_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1580_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1580_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1269_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1269_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1269_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1269_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1269_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1640_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1640_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1640_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1640_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1640_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1324_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1324_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1324_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1324_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1324_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1743_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1743_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1743_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1743_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_1743_gt.jpg} \\
    
    

==> rebuttal/synthesize_samples1.tex <==

    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0074_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0074_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0074_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0074_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0074_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0640_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0640_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0640_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0640_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0640_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0082_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0082_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0082_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0082_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0082_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0658_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0658_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0658_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0658_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0658_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0664_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0664_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0664_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0664_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0664_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0182_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0182_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0182_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0182_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0182_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0712_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0712_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0712_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0712_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0712_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0286_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0754_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0754_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0754_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0754_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0754_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0295_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0790_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0790_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0790_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0790_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0790_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0308_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0865_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0865_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0865_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0865_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0865_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0467_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0467_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0467_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0467_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0467_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0946_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0946_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0946_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0946_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0946_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0497_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0497_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0497_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0497_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0497_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0972_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0972_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0972_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0972_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0972_gt.jpg} \\
    
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0605_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0605_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0605_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0605_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0605_gt.jpg} &
    
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0983_image.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0983_bdrar.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0983_dsdnet.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0983_ours.jpg} &
    \includegraphics[width=0.10\linewidth]{rebuttal/synthesize/USR_shadow_free_0983_gt.jpg} \\
    
    

==> revision/synthesize_part_tiny.tex <==

    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0002_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0004_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0008_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0014_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0018_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0023_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0029_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0030_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0033_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0043_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0052_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0055_gt.jpg} \\
    
    %%%
    
     
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0169_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0177_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0181_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0184_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0188_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0194_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0202_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0212_gt.jpg} \\
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0224_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0227_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0229_gt.jpg} &
    
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_image.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_ours.jpg} &
    \includegraphics[width=0.08\linewidth]{rebuttal/synthesize/USR_shadow_free_0239_gt.jpg} \\
